The Detection and Characterization of cm Radio Continuum Emission from the Low-mass Protostar L1014-IRS

Observations by the Cores to Disk Legacy Team with the Spitzer Space Telescope have identified a low luminosity, mid-infrared source within the dense core, Lynds 1014, which was previously thought to harbor no internal source. Followup near-infrared and submillimeter interferometric observations have confirmed the protostellar nature of this source by detecting scattered light from an outflow cavity and a weak molecular outflow. In this paper, we report the detection of cm continuum emission with the VLA. The emission is characterized by a quiescent, unresolved 90 uJy 6 cm source within 0.2" of the Spitzer source. The spectral index of the quiescent component is $\alpha = 0.37\pm 0.34$ between 6 cm and 3.6 cm. A factor of two increase in 6 cm emission was detected during one epoch and circular polarization was marginally detected at the $5\sigma$ level with Stokes {V/I} $= 48 \pm 16$% . We have searched for 22 GHz H2O maser emission toward L1014-IRS, but no masers were detected during 7 epochs of observations between June 2004 and December 2006. L1014-IRS appears to be a low-mass, accreting protostar which exhibits cm emission from a thermal jet or a wind, with a variable non-thermal emission component. The quiescent cm radio emission is noticeably above the correlation of 3.6 cm and 6 cm luminosity versus bolometric luminosity, indicating more radio emission than expected. We characterize the cm continuum emission in terms of observations of other low-mass protostars, including updated correlations of centimeter continuum emission with bolometric luminosity and outflow force, and discuss the implications of recent larger distance estimates on the physical attributes of the protostar and dense molecular core.

==> commands.tex <==
% General purpose macros
\newcommand{\ee}[1]{\mbox{${} \times 10^{#1}$}}% scientific number format
\newcommand{\eten}[1]{\mbox{$10^{#1}$}}% power of ten

%macros for RA and Dec
%\newcommand{\h}{\mbox{{$^h$}}
%\newcommand{\m}{\mbox{{$^m$}}
%\newcommand{\s}{\mbox{{$^s$}}
\newcommand{\degree}{\mbox{$^{\circ}$}}
\newcommand{\am}{\mbox{\arcmin}}
\newcommand{\as}{\mbox{\arcsec}}

%macros for distance, volume, speed
\newcommand{\kms}{\mbox{km s$^{-1}$}}% km/s
\newcommand\cmv{\mbox{cm$^{-3}$}}
\newcommand\cmc{\mbox{cm$^{-2}$}}
\newcommand\cmdv{\mbox{cm$^{-2}$ (\kms)$^{-1}$}}
\newcommand{\um}{$\mu$m}
\newcommand{\micron}{$\mu$m}

%macros for references
\newcommand{\apj}{ApJ}
\newcommand{\apjs}{ApJS}
\newcommand{\mnras}{MNRAS}
\newcommand{\apjl}{ApJL}
\newcommand{\aap}{A\&A}

%macros for commonly used symbols
\newcommand{\x}{\mbox{${}\times{}$}}
\def\lsim {$\rlap{\raise.4ex\hbox{$<$}}\lower.55ex\hbox{$\sim$}\,$}
\def\to {$\rightarrow$}
\def\about {$\sim$}

%macros to avoid typing headache and needless acronyms simultaneously
\newcommand{\iras}{\mbox{\it IRAS}}
\newcommand{\iso}{\mbox{\it ISO}}
\newcommand{\mm}{millimeter}
\newcommand\submm{submillimeter}
\newcommand\smm{submillimeter}
\newcommand\fir{far-infrared}
\newcommand\mir{mid-infrared}
\newcommand\nir{near-infrared}
\newcommand{\sfr }{\mbox{$\dot M_{\star}$}}
\newcommand\sed{spectral energy distribution}
\newcommand{\lsun}{\mbox{L$_\odot$}}% Lsun
\newcommand{\msun}{\mbox{M$_\odot$}}% Msun
\newcommand{\ta}{{$T_A^*$}}
\newcommand{\tex}{\mbox{$T_{\rm ex}$}}
\newcommand{\tmb}{\mbox{$T_{\rm mb}$}}
\newcommand{\tr}{\mbox{$T_R$}}
\newcommand{\tk}{\mbox{$T_K$}}
\newcommand{\td}{\mbox{$T_d$}}
\newcommand{\lbol}{\mbox{$L_{bol}$}} % bolometric luminosity
\newcommand{\tbol}{\mbox{$T_{bol}$}} % bolometric temperature
\newcommand{\n}{\mbox{$n$}}
\newcommand{\nbar}{\mbox{$\overline{n}$}}
\newcommand{\nc}{\mbox{$n_c(jk)$}}
\newcommand{\mc}{\mbox{$M_N$}} % column density mass
\newcommand{\mn}{\mbox{$M_n$}} % density mass
\newcommand{\meanl}{\mbox{$\langle l \rangle$}} % mean size
\newcommand{\meanar}{\mbox{$\langle a/b \rangle$}} % mean aspect ratio
\newcommand{\mean}[1]{\mbox{$\langle#1\rangle$}} %generic mean for defined qu.
\newcommand{\opacity}{\mbox{$\kappa(\nu)$}} % opacity as func. of freq.
\newcommand{\av}{\mbox{$A_V$}} % Visual Extinction
\newcommand{\bperp}{\mbox{$B_{\perp}$}} % Projection of B on plane of sky
\newcommand{\rinf}{\mbox{$r_{inf}$}} % infall radius
\newcommand{\fsmm}{\mbox{$L_{smm}/L_{bol}$}} % submm lum over bol. luminosity
\newcommand{\lsmm}{\mbox{$L_{smm}$}} % luminosity longward of 350 mic.
\newcommand{\alphanir}{\mbox{$\alpha_{NIR}$}} % spectral index 2-20 mic.
 
%macros for molecule names
\newcommand{\hh}{\mbox{{\rm H}$_2$}}
\newcommand{\form}{H$_2$CO}
\newcommand{\water}{H$_2$O}
\newcommand{\ammonia}{\mbox{{\rm NH}$_3$}}
\newcommand{\coo}{$^{13}$CO}
\newcommand{\cooo}{C$^{18}$O}
\newcommand{\coooo}{C$^{17}$O}
\newcommand{\hcop}{HCO$^+$}
\newcommand{\hcopi}{H$^{13}$CO$^+$}
\newcommand{\dcop}{DCO$^+$}
\newcommand{\nthp}{N$_2$H$^+$}
\newcommand{\cs}{C$^{32}$S}
\newcommand{\css}{C$^{34}$S}
\newcommand{\HII}{\mbox{{\rm H}\,{\scriptsize II}}}


%macros for molecular transitions
\newcommand{\csfifo}{C$^{32}$S $J = 5 \rightarrow 4$}
\newcommand{\cssfifo}{C$^{34}$S $J = 5 \rightarrow 4$}
\newcommand{\cssesi}{C$^{32}$S $J = 7 \rightarrow 6$}
 
%%% macros for figures in postscript format
%   syntax: \psfig{vertical size}{ps file name}{caption}
%\input{epsf}
%\newcommand{\psfig}[3]
%           {{\begin{figure}[tbp]
%             \vbox to#1{\epsfxsize=\textwidth\epsfbox{#2.ps}}
%             \caption{#3}
%             \end{figure}}}
%\newcommand{\psscaledfig}[4]
%           {{\begin{figure}[tbp]
%             \centerline{\vbox to#1{\epsfxsize=#2\epsfbox{#3.ps}}}
%             \caption{#4}
%             \end{figure}}}
 















